Symetra: Visual Analytics for the Parameter Tuning Process of Symbolic Execution Engines

Symbolic execution engines such as KLEE automatically generate test cases to maximize branch coverage, but their numerous parameters make it difficult to understand the parameters' impact, leading the user to rely on suboptimal default configurations. While automated tuners have shown promising results, they provide limited insights into why certain configurations work well, motivating the need for Human-in-the-Loop approaches. In this work, we present a visual analytics system, Symetra, designed to support Human-in-the-Loop parameter tuning of symbolic execution engines. To handle a large number of parameters and their configurations, we provide two complementary overviews of their impact on branch coverage values and patterns. Building on these overviews, our system enables collective analysis, allowing the user to contrast groups of configurations and identify differences that may affect branch coverage. We also report on case studies and a Human-in-the-Loop tuning process, demonstrating that experts not only interpreted parameter impacts and identified complementary configurations, but also improved upon fully automated approaches in both branch coverage and tuning efficiency.

==> sections/05-04-discussion.tex <==

\subsection{Discussion}
% \tocheck{
% (specific)

% 정해진 시간동안 기다려야하는 -> 리얼타임/인터렉티프하게 할려고 하는게 쉽지 않다. 
% KLEE는 CLI 툴,
% 파라미터가 몇개 없는 녀석 -> 인터렉티브 시스템이 있는데
% 많은 애들에 대해서는 
% 파라미터의 영향을 오버뷰로 보여주는게 중요하지만, 어떤 무언가.. 

% 비슷한 패턴/유의미한 사용자가 시멘틱한 그룹을 만들어서 효과를 비교할 수 있게 해라 
% 기존 애들은 수백개, scalability해소 ->



% 우리가 DR을 한게 hp 에서 한게 아니고 (기존은 hp에서 함), 브랜치로 함
% -> 그걸 강조하는 게 좋지 않을까?

% familiarity가 중요하다 / node link diagram -> VA가 처음인 사람들은 친숙한게 중요하다. (bar 차트 등)

% 1. VA가 국한되어있는데, 넓혀보자. default를 믿지 마라-> 생각보다 사람들은 무작정 쓴다. 그거가 이 분야에서는 10년 넘게 썼다, 디폴트가 안좋은지 몰랐다 VA가 이걸 확장할 수 있는 영역이다. (Overtrust)

% }

\edit{Our evaluations demonstrate that \system enables experts to understand parameter impacts and identify complementary configurations. The optimization experiment shows that these insights translate to measurable improvements, achieving comparable coverage in one hour compared to 27 hours for the fully automated approach.

Beyond validating system utility, our study reveals two broader implications. First, the user often overtrusts default configurations. In our optimization experiment, switching from KLEE's defaults to program-specific values improved accumulated coverage by 17.5\%. These defaults have been used for over a decade without systematic examination, and visual analytics can expose such hidden assumptions by making parameter effects transparent.

Second, projecting trials by branch coverage vectors, rather than by parameter values, proved effective for identifying complementary configurations. Prior HPO visualization systems apply dimensionality reduction to parameter configurations, but \system projects by branch coverage vectors, enabling discovery of complementary configurations while addressing scalability.
}
% Throughout the case studies, both experts appreciated \system's capabilities.
% P1 valued the ability to visualize branch coverage vectors across trial groups, which are not discernible from aggregate coverage values alone, while P2 appreciated the support for analyzing potential causes of failures.
% \edit{Throughout the case studies, both experts leveraged \system's coordinated views to accomplish distinct analytical goals.
% P1 used the Coverage View's projection to discover complementary search strategies that were not discernible from aggregate coverage values alone, while P2 utilized the Parameter View's effect breakdown to systematically diagnose failure causes.
% Both case studies demonstrated how the drill-down workflow, from overview (Parameter and Coverage Views) to detailed comparison (Comparison and Code Views), enabled experts to not only identify patterns but also verify their underlying causes at the source code level.
% }

% Post-study interviews revealed that both participants found the Comparison and Code Views most useful for comparative analysis between groups to identify strategies for improving branch coverage (\textbf{G2}), replacing manual and time-consuming analysis.
% P1 highlighted the workflow streamlined by the Code View: \textit{``Previously, analyzing covered branches required at least three separate steps: 1) identifying the branch ID, 2) locating the file and line number, and 3) opening the source in a code editor. 
% \system reduces this to a single integrated process.''} 
% \edit{They also emphasized the Parameter View's utility for understanding configuration impacts (\textbf{G1}).}
% They also emphasized the utility of the Parameter View in that it allowed them to understand the configurations' impact on branch coverage by quantifying the effect of the parameter and its values (\textbf{G1}). 

% Our case studies also reveal that the effectiveness of configurations varied significantly across different program structures.
% For \texttt{gcal}, the number of maximum forks (MF) had the greatest impact on branch coverage, whereas in \texttt{grep}, the choice of seed file (SF) was most important, likely due to the characteristic of the target program that branch coverage relies on regular expression patterns.
% This finding aligns with our initial motivation: default parameter values are often suboptimal, and understanding parameter configurations during the tuning process can offer insights for improving branch coverage.


% P2, who has experience as both a researcher and a developer in the software testing domain, noted that the system would be useful in two distinct contexts.
% As a researcher aiming to increase branch coverage, he would use the system to identify effective parameter values and guide the tuner in prioritizing them.
% He also commented that the system is useful for developers tasked with testing specific source files, as it enables them to identify the parameters that cover those files, fix those parameters, and experiment with others to improve overall coverage.
% \tocheck{Implication of our study: 2개 정도 / 뭘 배웠는지 / }

% The expert feedback also highlighted areas for improvement.
% Both participants requested enhanced filtering capabilities in the Trial View beyond the current sorting functionality. 
% P1 suggested adding filters to create groups with specific attributes, while P2 emphasized the need to view only trials meeting certain criteria. 
% Furthermore, the experts proposed a tighter integration between the \system and the KLEE engine. This integration would enable them to run the KLEE engine directly from the interface to test parameter configurations identified as promising. 
% Additionally, P2 suggested implementing a backward tracing feature, allowing the user to select a code line and automatically identify configurations that cover it, which would be particularly useful for developers who are more interested in testing certain lines of code.





==> sections/06-use-case.tex <==


\subsection{Optimization in Practice}
% \section{Human-in-the-Loop Parameter Tuning}


% The case study results motivated us to explore how the insights gained from \system could be leveraged to enhance branch coverage. Specifically, we examined the extent to which such a Human-in-the-Loop tuning process (i.e., tuner and \system) can outperform a fully automated approach (i.e., tuner-only).
% E1 and E2, who participated in the design study, were tasked with using our system to analyze the results of an initial tuner run and refine the parameter space to improve branch coverage.
% After they adjusted the parameter space, we re-ran the experiment to assess whether branch coverage had improved. This process was repeated over three iterations.
\edit{We examined whether Human-in-the-Loop tuning (i.e., tuner and \system) can outperform a fully automated approach (i.e., tuner-only).
E1 and E2 were tasked with using our system to analyze the results of an initial tuner run and refine the parameter space to improve branch coverage. 
After adjusting the parameter space, we re-ran the experiment to assess whether branch coverage had improved. This process was repeated over three iterations.
We used \texttt{gawk} ($N_B=10,720$) as the target program with SymTuner~\cite{10.1145/3510003.3510185}, generating 800 trials per experiment (27 hours each).
We measured three metrics: $Acc_{800}$ (the accumulated coverage of all trials), $N_{failed}$ (the number of failed trials), and $Acc_{30}$ (the accumulated coverage of the first 30 trials to capture how quickly the tuner achieves good coverage when starting from better initial configurations).
The initial experiment with default parameters achieved $Acc_{800}=3,832$, $N_{failed}=128$, and $Acc_{30}=3,411$.
}


% We chose \texttt{gawk} ($N_B=10,720$) as the target program and used SymTuner~\cite{10.1145/3510003.3510185} to generate and evaluate 800 trials in each experiment, which took about 27 hours per experiment.
% We measured three metrics to evaluate each experiment: 1) $Acc_{800}$, the accumulated branch coverage value of all 800 trials (higher is better), 2) $N_{failed}$, the number of the failed trials having a branch coverage value of zero (lower is better), and 3) $Acc_{30}$ the accumulated branch coverage value of the first 30 trials (higher is better).
% We included $Acc_{30}$ to capture how quickly the tuner achieves good coverage when starting from better initial configurations.
% For the initial experiment, we used the default parameter space ($N_P=61$), as in the case studies.
% The initial experiment achieved $Acc_{800}=3,832$, $N_{failed}=128$, and $Acc_{30}=3,411$.

\paragraph*{Filtering Out Parameters with Little Effects.}
In the first iteration, while examining the Parameter View, the experts chose to exclude 28 parameters whose average effect on branch coverage was below 0.3.
They also noticed the parameters with values outperforming the default, highlighted by red dots in the Parameter View, and adjusted their defaults to the values with the greatest positive effect.
After the refinement, they achieved $Acc_{800}=4,093$ (6.8\% $\uparrow$), $N_{failed}=22$ (82.8\% $\downarrow$), and $Acc_{30}=3,651$ (7.0\% $\uparrow$).
This demonstrates that program-specific defaults enable faster convergence and higher coverage.


\paragraph*{Removing the Parameter Values Commonly Used in the Failed Trials.}
In the second iteration, they created a trial group of the 22 failed runs (i.e., $C_i=0$) through the Trial View.
Inspecting the histograms of parameter values in the Comparison View, they identified four common parameter values used in the group, which they believed to lead to failures: KCO=\val{true}, ST=\val{llvm}, DI=\val{true}, and DV=\val{false}. 
After excluding those values, they achieved $Acc_{800}=4,379$ (7.0\% $\uparrow$), $N_{failed}=0$ (100\% $\downarrow$), and $Acc_{30}=3,704$ (1.5\% $\uparrow$).
This demonstrates that incorporating user engagement into automated tuning can enhance both the efficiency and the reliability of the tuning process.


\paragraph*{Redefining the Defaults.}
In the third iteration, they found out that there were 16 parameters with a better default (i.e., with the red dots) in the Parameter View, while they changed the defaults in the first iteration.
Considering the interaction effect of the changes made in the second iteration, they adjusted the defaults of the 16 parameters to the values that demonstrated the greatest positive effect.
After the third refinement, they finally achieved $Acc_{800}=4,502$ (2.8\% $\uparrow$), $N_{failed}=0$ (no change), and $Acc_{30}=3,813$ (2.9\% $\uparrow$).

\edit{After three iterations, Human-in-the-Loop tuning achieved coverage of 3,813 within one hour. This is comparable to 3,832 obtained by the automated approach in 27 hours, demonstrating significant improvements in both coverage and efficiency.
}
% Through three experiments, each building on the improvements of the previous one, we observed how the insights provided by our system can be leveraged to enhance both branch coverage and testing efficiency. Notably, after three iterations, we achieved a coverage value of 3,813 within one hour—comparable to the final value of 3,832 obtained without refinement, which required approximately 27 hours—demonstrating the potential of Human-in-the-Loop parameter tuning.

% 제거한 파라미터들
% all-external-warnings
% watchdog
% batch-time
% uncovered-update-interval
% cex-cache-superset
% warnings-only-to-file
% const-array-opt
% max-forks
% klee-call-optimisation
% emit-all-errors
% max-solver-time
% seed-time
% use-independent-solver
% return-null-on-zero-malloc
% use-visitor-hash
% max-sym-array-size
% zero-seed-extension
% track-instruction-time

